Precision angular diameters for 16 southern stars with VLTI/PIONIER

In the current era of Gaia and large, high signal to noise stellar spectroscopic surveys, there is an unmet need for a reliable library of fundamentally calibrated stellar effective temperatures based on accurate stellar diameters. Here we present a set of precision diameters and temperatures for a sample of 6 dwarf, 5 sub-giant, and 5 giant stars observed with the PIONIER beam combiner at the VLTI. Science targets were observed in at least two sequences with five unique calibration stars each for accurate visibility calibration and to reduce the impact of bad calibrators. We use the standard PIONIER data reduction pipeline, but bootstrap over interferograms, in addition to employing a Monte-Carlo approach to account for correlated errors by sampling stellar parameters, limb darkening coefficients, and fluxes, as well as predicted calibrator angular diameters. The resulting diameters were then combined with bolometric fluxes derived from broadband Hipparcos-Tycho photometry and MARCS model bolometric corrections, plus parallaxes from Gaia to produce effective temperatures, physical radii, and luminosities for each star observed. Our stars have mean angular diameter and temperatures uncertainties of 0.8% and 0.9% respectively, with our sample including diameters for 10 stars with no pre-existing interferometric measurements. The remaining stars are consistent with previous measurements, with the exception of a single star which we observe here with PIONIER at both higher resolution and greater sensitivity than was achieved in earlier work.

==> tables/table_calibrators.tex <==
\begin{tabular}{cccccc}
\hline
HD & SpT & VTmag & Hmag & Quality & Target/s \\
 &  & (mag) & (mag) &  &  \\
\hline
HD9228 & K2III & 6.08 & 3.131 & ... & TauCet\\
HD10148 & F0V & 5.612 & 4.832 & nan & TauCet\\
HD18978 & A3IV-V & 4.092 & 3.539 & nan & TauCet\\
HD17206 & F7V & 4.521 & 3.236 & nan & TauCet\\
HD18622 & nan & nan & nan & BAD & TauCet, alfHyi, chiEri\\
HD1581 & F9.5V & 4.286 & 2.738 & nan & alfHyi, chiEri\\
HD15233 & F2II/III & 5.4 & 4.515 & nan & alfHyi\\
HD19319 &  F0III/IV & 5.163 & 4.275 & nan & alfHyi\\
HD11332 & K0III & 6.251 & 3.705 & nan & alfHyi, chiEri\\
HD10019 & G8III & 6.95 & 4.76 & nan & chiEri\\
HD16970 & nan & nan & nan & BAD & 95Cet, delEri, epsEri\\
HD19866 & K0III & 7.209 & 4.728 & nan & 95Cet\\
HD20699 & K0III & 6.835 & 4.746 & nan & 95Cet\\
HD19994 & F8.5V & 5.135 & 3.768 & nan & 95Cet\\
HD22484 & F9IV-V & 4.353 & 2.916 & nan & 95Cet, omi2Eri\\
HD21530 & K2II/III & 5.854 & 3.329 & nan & epsEri\\
HD25725 & M7+II & 8.745 & -0.318 & nan & epsEri\\
HD20010A & F6V & 3.976 & 2.317 & CHECK & delEri, epsEri\\
HD24555 & G6.5III & nan & nan & CHECK & delEri, epsEri\\
HD23304 & K0III & 7.331 & 4.881 & nan & delEri\\
HD26464 & K1III & 5.807 & 3.546 & ... & delEri, omi2Eri\\
HD24780 & K4/5III & 8.492 & 4.84 & nan & omi2Eri\\
HD26409 & G8III & 5.546 & 3.588 & nan & omi2Eri\\
HD27487 & G8III & 6.826 & 4.751 & nan & omi2Eri\\
HD33111 & A3IV & 2.779 & 2.439 & nan & omi2Eri\\
HD136498 & K2III & 7.895 & 4.674 & nan & 37Lib\\
HD139155 & K2/3IV & 8.637 & 4.996 & nan & 37Lib\\
HD149757 & O9.2IVnn & 2.546 & 2.667 & nan & 37Lib\\
HD132052 & F2V & 4.503 & 3.824 & nan & 37Lib\\
HD141795 & kA2hA5mA7V & 3.714 & 3.44 & nan & 37Lib\\
HD128898 & A7VpSrCrEu & 3.189 & 2.471 & nan & betTrA\\
HD140018 & K1/2III & 7.01 & 3.97 & nan & betTrA\\
HD143853 & K1III & 7.238 & 3.917 & nan & betTrA\\
HD136225 & K3III & 7.302 & 3.658 & nan & betTrA\\
HD165040 & kA4hF0mF2III & 4.359 & 3.804 & nan & HR7221, betTrA\\
HD166464 & K0III & 5.081 & 2.715 & nan & lamSgr\\
HD167720 & K2III & 5.974 & 2.427 & nan & lamSgr\\
HD175191 & B2V & nan & nan & BAD & lamSgr\\
HD165634 & G7:IIIbCN-1CH-3.5HK+1 & 4.661 & 2.19 & nan & lamSgr\\
HD169022 & B9.5III & nan & nan & CHECK & lamSgr\\
HD184574 & K0III & 6.393 & 3.857 & nan & HD187289\\
HD187195 & K2III & 6.129 & 3.386 & nan & HD187289\\
HD187532 & F5VFe-1CH-0.7 & 5.425 & 4.625 & nan & HD187289\\
HD184835 & K0III & 5.782 & 2.918 & nan & HD187289\\
HD193896 & G5IIIa & 6.384 & 3.938 & nan & HD187289\\
HD192531 & K0III & 6.396 & 3.853 & nan & delPav\\
HD197051 & A7III & 3.431 & 2.794 & nan & delPav, epsInd\\
HD197359 & K0/1III & 6.822 & 4.47 & nan & delPav\\
HD169326 & K2III & 6.095 & 3.496 & nan & delPav\\
HD191937 & K3III & 6.719 & 3.574 & nan & delPav\\
HD205935 & K0II/III & 6.446 & 3.947 & nan & epsInd\\
HD209952 & B6V & nan & nan & CHECK & epsInd\\
HD212878 & G8III & 6.98 & 4.814 & nan & epsInd\\
HD219571 & F4V & 4.033 & 3.077 & nan & epsInd\\
HD4188 & K0III & 4.878 & 2.669 & nan & TauCet\\
HD129008 & G8III/IV & 7.251 & 4.879 & nan & HD131977\\
HD133649 & K0III & 7.813 & 4.96 & nan & HD131977\\
HD133670 & K0III & 6.247 & 3.827 & nan & HD131977\\
HD129502 & F2V & 3.907 & 3.069 & nan & HD131977\\
HD133627 & K0III & 6.862 & 4.335 & nan & HD131977\\
HD152236 &  B1Ia-0ek & 4.817 & 3.341 & BAD & etaSco\\
HD152293 & F3II & 5.91 & 4.251 & nan & etaSco\\
HD158408 & B2IV & 2.624 & 3.108 & BAD & etaSco\\
HD135382 & A1V & 2.849 & 2.527 & nan & etaSco\\
HD160032 & F4V & 4.799 & 3.702 & nan & etaSco\\
HD182835 & F2Ib & 4.729 & 2.866 & nan & betAql\\
HD193329 & K0III & 6.164 & 3.826 & nan & betAql\\
HD189533 & G8II & 6.845 & 3.743 & nan & betAql\\
HD189188 & K2III & 6.895 & 3.735 & nan & betAql\\
HD194013 & G8III-IV & 5.409 & 3.31 & nan & betAql\\
HD172555 & A7V & 4.793 & 4.251 & nan & HR7221\\
HD173948 & B2Ve & 4.181 & 4.318 & nan & HR7221\\
HD161955 & K0/1III & 6.582 & 4.102 & nan & HR7221\\
HD188228 & A0Va & 3.938 & 3.762 & nan & HR7221, gamPav\\
HD208937 & K0III & 7.493 & 4.941 & nan & gamPav\\
HD212211 & F5III & 5.814 & 4.895 & nan & gamPav\\
HD186219 & A4IV & 5.422 & 4.888 & nan & gamPav\\
HD217831 & F3III & 5.56 & 4.87 & nan & gamPav\\
HD110335 & B5III & 4.904 & 4.933 & nan & ProximaCen\\
HD125158 & A5/7mA7-F2 & 5.242 & 4.788 & nan & ProximaCen\\
HD125288 & B5Ib/II & 4.347 & 4.154 & nan & ProximaCen\\
HD133869 & K3III & 8.211 & 3.718 & nan &\\
HD128398 & F7IV & 6.593 & 5.375 & nan &\\
HD128917 & F5V & 6.256 & 5.161 & nan &\\
\hline
\end{tabular}


==> tables/table_fbol_2.tex <==
\begin{tabular}{cccc}
\hline
Star & HD & f$_{\rm bol}$ (MARCS) & $\sigma_{f_{\rm bol}} (\zeta)$ \\
 &  & (10$^{-8}\,$ergs s$^{-1}$ cm $^{-2}$) & (\%) \\
\hline
40 Eri A & 26965 & H$_p$: 51.806 & 0.95 \\
 & & B$_T$: 50.183 &2.61 \\
 & & V$_T$: 52.198 &1.31 \\
 & & B$_P$: 52.194 &1.12 \\
 & & R$_P$: 54.415 &0.30 \\
37 Lib & 138716 & H$_p$: 50.064 & 3.01 \\
 & & B$_T$: 51.696 &6.75 \\
 & & V$_T$: 50.461 &3.57 \\
 & & B$_P$: 50.687 &3.32 \\
 & & R$_P$: 50.829 &0.77 \\
$\beta$ TrA & 141891 & H$_p$: 187.705 & 0.81 \\
 & & B$_T$: 189.025 &1.62 \\
 & & V$_T$: 189.973 &1.18 \\
 & & B$_P$: 7.880 &37.06 \\
 & & R$_P$: 179.156 &1.15 \\
$\lambda$ Sgr & 169916 & H$_p$: 273.951 & 1.80 \\
 & & B$_T$: 288.615 &4.03 \\
 & & V$_T$: 279.522 &2.24 \\
 & & B$_P$: 139.938 &14.51 \\
 & & R$_P$: 201.411 &1.67 \\
$\delta$ Pav & 190248 & H$_p$: 105.636 & 0.97 \\
 & & B$_T$: 110.851 &2.99 \\
 & & V$_T$: 106.716 &1.31 \\
 & & B$_P$: 91.156 &2.40 \\
 & & R$_P$: 104.679 &0.41 \\
$\epsilon$ Ind & 209100 & H$_p$: 51.824 & 4.41 \\
 & & B$_T$: 50.943 &8.88 \\
 & & V$_T$: 52.171 &5.34 \\
 & & B$_P$: 52.938 &4.81 \\
 & & R$_P$: 53.268 &0.93 \\
HD131977 & 131977 & H$_p$: 18.617 & 4.91 \\
 & & B$_T$: 16.958 &8.41 \\
 & & V$_T$: 18.431 &5.05 \\
 & & B$_P$: 18.669 &4.51 \\
 & & R$_P$: 20.196 &0.89 \\
$\eta$ Sco & 155203 & H$_p$: 120.660 & 0.96 \\
 & & B$_T$: 121.859 &2.26 \\
 & & V$_T$: 121.613 &1.32 \\
 & & B$_P$: 106.332 &1.89 \\
 & & R$_P$: 117.687 &1.09 \\
$\beta$ Aql & 188512 & H$_p$: 100.453 & 1.47 \\
 & & B$_T$: 99.957 &3.89 \\
 & & V$_T$: 101.166 &1.81 \\
 & & B$_P$: 95.363 &1.95 \\
 & & R$_P$: 102.234 &0.80 \\
HR7221 & 177389 & H$_p$: 25.459 & 1.74 \\
 & & B$_T$: 28.680 &3.94 \\
 & & V$_T$: 25.927 &2.14 \\
 & & B$_P$: 26.043 &1.93 \\
 & & R$_P$: 24.143 &0.40 \\
\hline
\end{tabular}


==> tables/table_observations_1.tex <==
\begin{tabular}{cccccc}
\hline
HD & UT Date & ESO & Sequence & Baseline & Calibrator \\
 &  & Period & Type &  & HD \\
\hline
epsInd & 2017-07-22 & 99 & faint & A0-G1-J2-K0 & 205935, 209952, 212878 \\
HD187289 & 2017-07-24 & 99 & faint & A0-G1-J2-K0 & 184574, 187195, 187532 \\
alfHyi & 2017-07-24 & 99 & faint & A0-G1-J2-K0 & 1581, 15233, 19319 \\
chiEri & 2017-07-24 & 99 & bright & A0-G1-J2-K0 & 1581, 11332, 18622 \\
37Lib & 2017-07-25 & 99 & faint & A0-G1-J2-K0 & 136498, 139155, 149757 \\
HD187289 & 2017-07-25 & 99 & bright & A0-G1-J2-K0 & 184835, 187195, 193896 \\
betTrA & 2017-07-25 & 99 & bright & A0-G1-J2-K0 & 128898, 136225, 165040 \\
alfHyi & 2017-07-26 & 99 & bright & A0-G1-J2-J3 & 1581, 11332, 18622 \\
chiEri & 2017-07-27 & 99 & faint & A0-G1-J2-J3 & 10019, 11332, 18622 \\
TauCet & 2017-08-17 & 99 & faint & A0-G1-J2-K0 & 9228, 10148, 18978 \\
epsInd & 2017-08-17 & 99 & bright & A0-G1-J2-K0 & 197051, 209952, 219571 \\
95Cet & 2017-08-26 & 99 & bright & A0-G1-J2-J3 & 16970, 19994, 22484 \\
TauCet & 2017-08-26 & 99 & bright & A0-G1-J2-J3 & 9228, 17206, 18622 \\
lamSgr & 2017-08-26 & 99 & faint & A0-G1-J2-J3 & 166464, 167720, 175191 \\
delPav & 2017-08-27 & 99 & faint & A0-G1-J2-J3 & 192531, 197051, 197359 \\
95Cet & 2017-09-01 & 99 & faint & A0-G1-J2-J3 & 16970, 19866, 20699 \\
epsEri & 2017-09-04 & 99 & faint & A0-G1-J2-J3 & 16970, 21530, 25725 \\
omi2Eri & 2017-09-04 & 99 & faint & A0-G1-J2-J3 & 24780, 26409, 27487 \\
epsEri & 2017-09-05 & 99 & bright & A0-G1-J2-J3 & 16970, 20010A, 24555 \\
lamSgr & 2017-09-08 & 99 & bright & A0-G1-J2-J3 & 165634, 169022, 175191 \\
delPav & 2017-09-12 & 99 & bright & A0-G1-J2-J3 & 169326, 197051, 191937 \\
delEri & 2017-09-24 & 99 & faint & A0-G1-J2-J3 & 16970, 23304, 26464 \\
betTrA & 2018-04-18 & 101 & faint & A0-G1-J2-J3 & 128898, 140018, 143853 \\
betAql & 2018-06-04 & 101 & bright & A0-G1-J2-J3 & 182835, 189188, 194013 \\
epsInd & 2018-06-04 & 101 & bright & A0-G1-J2-J3 & 197051, 209952, 219571 \\
HD131977 & 2018-06-05 & 101 & faint & A0-G1-J2-J3 & 129008, 133649, 133670 \\
HR7221 & 2018-06-05 & 101 & bright & A0-G1-J2-J3 & 161955, 165040, 188228 \\
HD131977 & 2018-06-06 & 101 & bright & A0-G1-J2-J3 & 129502, 133627, 133670 \\
HR7221 & 2018-06-06 & 101 & faint & A0-G1-J2-J3 & 165040, 172555, 173948 \\
epsInd & 2018-06-06 & 101 & faint & A0-G1-J2-J3 & 205935, 209952, 212878 \\
\hline
\end{tabular}


==> tables/table_observations_2.tex <==
\begin{tabular}{cccccc}
\hline
HD & UT Date & ESO & Sequence & Baseline & Calibrator \\
 &  & Period & Type &  & HD \\
\hline
etaSco & 2018-06-06 & 101 & bright & A0-G1-J2-J3 & 135382, 158408, 160032 \\
etaSco & 2018-06-07 & 101 & faint & A0-G1-J2-J3 & 152236, 152293, 158408 \\
TauCet & 2018-08-06 & 101 & bright & A0-G1-J2-J3 & 4188, 9228, 17206 \\
TauCet & 2018-08-07 & 101 & faint & A0-G1-J2-J3 & 9228, 10148, 18978 \\
betTrA & 2018-08-07 & 101 & bright & A0-G1-J2-J3 & 128898, 136225, 165040 \\
delEri & 2018-11-25 & 102 & bright & A0-G1-J2-J3 & 16970, 20010A, 24555 \\
delEri & 2018-11-26 & 102 & faint & A0-G1-J2-J3 & 16970, 23304, 26464 \\
omi2Eri & 2018-11-26 & 102 & bright & A0-G1-J2-J3 & 26409, 26464, 33111 \\
\hline
\end{tabular}

